Inferring Message Flows From System Communication Traces

This paper proposes a novel method for automatically inferring message flow specifications from the communication traces of a system-on-chip (SoC) design that captures messages exchanged among the components during a system execution. The inferred message flows characterize the communication and coordination of components in a system design for realizing various system functions, and they are essential for SoC validation and debugging. The proposed method relieves the burden of manual development and maintenance of such specifications on human designers. Our method also uses a new accuracy metric, \emph{acceptance ratio}, to evaluate the quality of the mined specifications instead of the specification size often used in the previous work, enabling more accurate specifications to be mined. Furthermore, this paper introduces the concept of essential causalities to enhance the accuracy of the message flow mining and accelerate the mining process. The effectiveness of the proposed method is evaluated on both synthetic traces and traces generated from executing several system models in GEM5. In both cases, the proposed method achieves superior accuracies compared to a previous approach. Additionally, this paper includes some practical use cases.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> Sections/Acknowledgement.tex <==

\section*{Acknowledgment}

% The preferred spelling of the word ``acknowledgment'' in America is without 
% an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
% G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
% acknowledgments in the unnumbered footnote on the first page.

% \section*{References}

% Please number citations consecutively within brackets \cite{b1}. The 
% sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
% number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
% the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

% Number footnotes separately in superscripts. Place the actual footnote at 
% the bottom of the column in which it was cited. Do not put footnotes in the 
% abstract or reference list. Use letters for table footnotes.

% Unless there are six authors or more give all authors' names; do not use 
% ``et al.''. Papers that have not been published, even if they have been 
% submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
% that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
% Capitalize only the first word in a paper title, except for proper nouns and 
% element symbols.

% For papers published in translation journals, please give the English 
% citation first, followed by the original foreign-language citation \cite{b6}.

==> Sections/DAC24-Review.tex <==
============================================================================ \\
DAC 2024 Reviews for Submission \#918\\
============================================================================ \\
 
Title: AutoFlow: Inferring Message Flows From System Communication Traces\\
Authors: Bardia Nadimi and Hao Zheng\\
 
 
============================================================================\\
                            REVIEWER \#1\\
============================================================================\\
 
---------------------------------------------------------------------------\\
Reviewer's Scores\\
---------------------------------------------------------------------------\\
\noindent  Clarity / Writing Style (1-5): 4\\
      Originality / Innovativeness (1-5): 3\\
    Impact of Ideas and/or Results (1-5): 2\\
            OVERALL RECOMMENDATION (1-5): 3\\
 
Summarize shortly the contributions of the paper in your own words.\\
---------------------------------------------------------------------------\\
This paper proposes an approach to understand and infer message dependencies from communication traces. 
Since concurrent systems may have interleaved communication that appear in the traces, it is not straightforward to determine such dependencies. 
To this end, the approach aims to understand the true causality by analysing multiple traces. 
The evaluation of the approach shows that it can outperform prior works.\\
---------------------------------------------------------------------------\\
 
 
Strengths\\
---------------------------------------------------------------------------\\
+ Important problem to understand message flows\\
+ Presentation is mostly understandable\\
---------------------------------------------------------------------------\\
 
 
Weaknesses\\
---------------------------------------------------------------------------\\
- The approach is described pretty abstract\\
- Relation to message sequence chart mining\\
- The impact of model learning is unclear\\
---------------------------------------------------------------------------\\
 
 
Main Discussion of Paper\\
---------------------------------------------------------------------------\\
- Overall, specification mining is an interesting topic and understanding the specification from communication traces might be useful for various things. From this angle, the paper targets a nice problem. However, what is not clear from the paper is the usage of these results and the approach appears quite abstract, hence, resembling methods from software domain. In the following, I will elaborate on these points. \\
 
- Firstly, the specification mining approach appears quite straightforward and abstract in the paper. There is hardly any difference from a generic message sequence mining approach for concurrent systems. For such a topic, there has been a number of solutions in the past two decades and the paper does not clearly position itself with respect to the broader works of message sequence chart mining. \\
 
- Secondly, the processor communication traces are much more complex and may have several tiny details that are important for the mining to work. However, it remains unclear from the approach how these details play a role for the effectiveness of these mining. The proposed approach is a very straightforward threshold check on dependencies arising from a node. It would be better if the approach clarifies how the trace was simplified/processed to construct the graph. \\
 
- Thirdly, it is unclear to me why a threshold is checked for the causality. I would assume if there is a true causality, then the order will always be preserved. Precisely, if A is causally dependent on B, shouldn't A always appear after B in the trace? \\
 
- Finally, the paper does not do much on how these models can be used. If a model is learned by mining the traces, how this model can help in testing/optimization any other use cases would be good to show.\\
---------------------------------------------------------------------------\\
 
 
Have a Question to Authors? (Optional)\\
---------------------------------------------------------------------------\\
How the proposed approach can be more effective in this context than general message sequence chart mining approaches?\\
---------------------------------------------------------------------------\\
 
 
 
============================================================================\\
                            REVIEWER \#2\\
============================================================================\\
 
---------------------------------------------------------------------------\\
Reviewer's Scores\\
---------------------------------------------------------------------------\\
\noindent Clarity / Writing Style (1-5): 3\\
      Originality / Innovativeness (1-5): 3\\
    Impact of Ideas and/or Results (1-5): 2\\
            OVERALL RECOMMENDATION (1-5): 2\\
 
Summarize shortly the contributions of the paper in your own words.\\
---------------------------------------------------------------------------\\
This paper proposes a framework to infer message flow specification from complex system traces. It proposes the idea of a causality graph and then selects a set of longest paths to cover most messages. The approach is evaluated using GEM5 and mined two flow specifications that are not in GEM5 documentation.\\
---------------------------------------------------------------------------\\
 
 
Strengths\\
---------------------------------------------------------------------------\\
+ The approach is evaluated on GEM5 with full system mode and mined flows that are not in GEM5 documentation.\\
---------------------------------------------------------------------------\\
 
 
Weaknesses\\
---------------------------------------------------------------------------\\
- Similarity with the existing work [17].\\
- Human effort is needed in the framework.\\
---------------------------------------------------------------------------\\
 
 
Main Discussion of Paper\\
---------------------------------------------------------------------------\\
As claimed in the paper, the user's experience seems to be very important, as claimed in Section V-D, to decide the accuracy threshold.\\
 
Table I and II are not explained well. It is not clear to me what these columns represent.  \\
 
There are many places that are similar to [17]. For example,\\
Fig. 2(b) --- Fig. 1(a) in [17] are exactly the same\\
Fig. 5(b) --- Fig. 8 (a) in [17] are exactly the same\\
First sentence in Section II "Specification mining aims to derive patterns from various artifacts"  --- First sentence in Section II in [17] "Specification mining aims to extract patterns from various artifacts." 
Many other places are similar, and there is no need to list all of them here.\\
---------------------------------------------------------------------------\\
 
 
 
============================================================================\\
                            REVIEWER \#3\\
============================================================================\\
 
---------------------------------------------------------------------------\\
Reviewer's Scores\\
---------------------------------------------------------------------------\\
\noindent Clarity / Writing Style (1-5): 4\\
      Originality / Innovativeness (1-5): 3\\
    Impact of Ideas and/or Results (1-5): 3\\
            OVERALL RECOMMENDATION (1-5): 4\\
 
Summarize shortly the contributions of the paper in your own words.\\
---------------------------------------------------------------------------\\
The paper proposes a method called autoFlows, which automatically infers messages from system wide transactions and communications of an SoC during design  execution. The main reason for this approach is to avoid manual extraction of messages which are very error prone. A quality metric was defined which measures how good the data that was mined from approach was. A refinement step also exists to make sure the desired accuracy is reached. The effectiveness of this approach was measured using synthetic and actual traces from gem5 and showed superior accuracy when compared to other methods.\\
---------------------------------------------------------------------------\\
 
 
Strengths\\
---------------------------------------------------------------------------\\
improved accuracy\\
development of a method that helps is complex SoC validation\\
auto mining of data from traces\\
---------------------------------------------------------------------------\\
 
 
Weaknesses\\
---------------------------------------------------------------------------\\
poor runtime performance\\
weak benchmarks\\
---------------------------------------------------------------------------\\
 
 
Main Discussion of Paper\\
---------------------------------------------------------------------------\\
The paper proposes a method called autoFlows, which automatically infers messages from system wide transactions and communications of an SoC during design  execution. The main reason for this approach is to avoid manual extraction of messages which are very error prone. A quality metric was defined which measures how good the data that was mined from approach was. A refinement step also exists to make sure the desired accuracy is reached. The effectiveness of this approach was measured using synthetic and actual traces from gem5 and showed superior accuracy when compared to other methods. This paper auto mines data from traces and shows improved accuracy in their methods over previous methods that helps in complex SoC validation.\\
---------------------------------------------------------------------------\\

==> Sections/ICCAD23-Comments.tex <==

ICCAD 2023 Reviews for Submission number 783\\
Title: A Mining Approach for Inferring Message Flows From System Communication Traces
Authors: Bardia Nadimi and Hao Zheng

\section{REVIEWER 1}

\subsection{Reviewer's Scores:}

\noindent Relevance to ICCAD (1-5): 4\\
Novelty of technical ideas (1-5): 3\\
Theoretically sound (1-5): 2\\
Practically useful (1-5): 4\\
Thoroughness of the research (1-5): 3\\
Clarity and language (1-5): 4\\
Overall Recommendation (1-5): 3\\

\subsection{Summary}
This paper presents a method for "specification mining", which is the process of extracting specifications from observable system data (e.g., execution traces or log-files).
Compared to previous work, the authors claim to have been the first to focus not on the size of the resulting model, but on the accuracy.
To this end, the authors define a new way of measuring this accuracy and perform experiments that compare their algorithm to previous work in the field.

\subsection{Strengths}
The paper has a clear structure, is well written and the information is presented cleary.
The proposed approach is convincingly shown to be relevant (in the related work section) and evaluated rather thoroughly.


\subsection{Weaknesses}
The theoretical background could be more fleshed out in my opinion.
Although the content is explained really well, I would have appreciated a more complex mined message flow as an example.


\subsection{Detailed Comments}
I would have appreciated a more thorough theoretical analysis of the results.
Specification mining seems to me like it has close connections to formal language theory (e.g., formal grammals and their corresponding accepting automatons).
I would have appreciated at least a mention of these connections.

Furthermore, I think the authors could have provided more clear examples of mined specifications that would not have been easy to describe a-priori (which is the claimed main advantage of specification mining).
I understand that the authors chose the given examples (like a memory read that was compared to the actual specification in the gem-5 documentation) so that readers can understand the problem and I agree that these examples are well chosen.
However, I would have liked an additional example of a mined message flow that is valid but also complex enough so that it is clear why manual specification could not have been done easily.

I think there is something wrong with the sentence: " [...] and finding all available paths in the causality graph in a linear time is not achievable due to the enormous size of the available paths." in Section IV A.
Maybe my understanding is wrong but I don't think that the size of the causality graph has any influence on whether computations on it (like extracting valid traces) fall into a specific complexity class.
Maybe the authors wanted to make a statement about the feasibility of the computation, which does depend on the absolute size of the graph.

Overall, the paper is sound work that seems to improve upon the state of the art in meaningful ways by exploring a different trade-off than the presented related work.
The paper does have some weak spots, that should be addressed.


\section{REVIEWER 2}

\subsection{Reviewer's Scores}
\noindent Relevance to ICCAD (1-5): 4\\
        Novelty of technical ideas (1-5): 4\\
               Theoretically sound (1-5): 4\\
                Practically useful (1-5): 2\\
      Thoroughness of the research (1-5): 3\\
              Clarity and language (1-5): 4\\
            Overall Recommendation (1-5): 3\\

\subsection{Summary}
This paper presents a method to mine traces of communication among SOC communication to automatically extract a model whose behaviour can cover the generated traces with an acceptable level of accuracy in an iterative process of creating/refining model and evaluating it.


\subsection{Strengths}
The paper is exceptionally well written. Very easy to read, even for a non-specialist in this field.
The idea also seems enticing, and the authors have reviewed the state of the art well and concretely pointed out the differentiation.
The experimental results are also OK, though I am not entirely convinced about synthetic traces.



\subsection{Weaknesses}
My principal problem with this work is how it is used in practice. To create a SOC design, even at the GEM5 level, one needs a specification to start with, even if this specification is almost always non-executable. 
Once the SOC design team has a specification, and the model, if I understood correctly, this method will mine the traces generated by the simulation and then derive a model of the SOC. This model abstracted as an FSM, will generate a trace that covers the REAL trace generated by the SOC design (SystemC or GEM5 etc).
And then what ? This model is obviously neither complete nor an exact match - the coverage at best can asymptotically reach the actual trace. How do I use this mined model?


\subsection{Detailed Comments}
This intriguing work is very well written and backed by decent experiments. I enjoyed reading it.

I am not an expert in mining models from communication traces. I have, however, architected a few real-life industrial SOCs. 
I can't figure out how this will help me improve my verification or validation strategy.
The end-user makes many critical decisions, like the confidence of support for nodes and edges. I could not see how the end-user knows what a reasonable threshold is.




\section{REVIEWER 3}

\subsection{Reviewer's Scores}

\noindent Relevance to ICCAD (1-5): 3\\
        Novelty of technical ideas (1-5): 3\\
               Theoretically sound (1-5): 4\\
                Practically useful (1-5): 2\\
      Thoroughness of the research (1-5): 3\\
              Clarity and language (1-5): 4\\
            Overall Recommendation (1-5): 3\\

\subsection{Detailed Comments}
The paper addresses the issue of system model reconstruction from monitored
message traces. Available approaches try to infer a FSA model of minimal size.
This paper aims at also achieving a certain required level of accuracy. This
novelty is, basically,  the content of section IV C and D.

The paper is quite well written and experiments show the intended improvement
in coverage. What the paper does not show is the way in which this really is
useful in any way.



\section{REVIEWER 4}

\subsection{Reviewer's Scores}
\noindent Relevance to ICCAD (1-5): 4\\
        Novelty of technical ideas (1-5): 2\\
               Theoretically sound (1-5): 3\\
                Practically useful (1-5): 2\\
      Thoroughness of the research (1-5): 4\\
              Clarity and language (1-5): 2\\
            Overall Recommendation (1-5): 3\\

\subsection{Summary}
The paper proposes a new method to infer spec model from communication traces of SoC design. The communication traces represent messages exchanged by different components during system execution. 
They evaluate the method using synthetic traces and real traces generated from GEM5 simulator.


\subsection{Strengths}
* This paper is solving an important and hard problem, which is build a model to represent sophisticated system protocols.
* The paper designs new metrics, new evaluation method and refinement algorithm to improve their results.


\subsection{Weaknesses}
* The writing needs to be improved. Many typos out there.
* The model constructed from only communication traces seem not sufficiently complete.


\subsection{Detailed Comments}
Please justify the model built by the communication traces are good enough to model very complex systems protocols of SoCs.



==> Sections/RelatedWorks.tex <==
\section{Related Works (Copied from TCAD)}
\label{sec:rel-workOrg}

% {\bf you can borrow most of the related work from our previous papers}

% \marginpar{Copied from TCAD paper}

Specification mining aims to extract patterns from various artifacts. 
A model-based approach \textit{Synoptic} \cite{Beschastnikh:2011:LEI:2025113.2025151} mines invariants from logs of sequential execution traces where concurrency is recorded in the partial order. It then generates an FSM that satisfies the mined invariants. 
\emph{Perracotta}~\cite{Yang:2006} is another software execution log analysis tool that mines temporal API rules.  It describes a chaining technique that can be used to find long sequential patterns.
The work \textit{BaySpec} \cite{Mrowca:2019:LTS:3316781.3317847} extracts LTL formulas from Bayesian networks trained with software traces. It requires traces to be clearly partitioned with respect to different functions.
%It is not restricted by some user-defined template, thus may produce many useful unknown patterns. 
For mining hardware traces, the approaches presented in~\cite{Li2010DAC,Hertz:2013:tcad,Danese:2015:vlsi-soc,Danese:2015:date,Danese:2017:dac} mine assertions from either gate-level representations~\cite{Li2010DAC}, or RTL models~\cite{Chang:2010:aspdac,Hertz:2013:tcad,Danese:2015:vlsi-soc,Danese:2015:date,Danese:2017:dac}.
The work in~\cite{Liu:2013} describes an assertion mining approach using episode mining from the simulation traces of transaction-level models.
Those approaches often lack support for finding longer patterns, thus not being able to find complex communication patterns involving multiple components.
A recent work~\cite{Ahmed:mine-msg-flow:2021} considers a similar problem as this paper, but it only mines sequential patterns.
%, not the models this paper tries to infer. 

Work in~\cite{Noc_fabrics} proposes a security property validation method focusing on the communication fabrics of an SoC. It builds a CFG for each IP in the SoC and explores connections between various CFGs efficiently for any given security property. This work takes system-level interaction into consideration and demonstrates that the communication fabrics could be a vital point for vulnerability. Therefore, understanding the fabric-level communication model is important for validation activities.

Our work falls under the category of model synthesis methods.  
The aim of model synthesis is to identify a model from system execution traces such that the resulting model can accept the input traces.
In~\cite{Heule:2013}, the deterministic finite automata inference based on the original evidence-driven state merging method~\cite{Lang:1998:EDSM} is extended and formulated as a graph coloring problem, which is then solved by a Boolean satisfiability solver.  Recently, \emph{Trace2Model} is introduced in~\cite{natasa2020} that learns non-deterministic finite automata (NFA) models from software execution traces using C bounded model checking technique. Similar work can also be found in~\cite{Ulyantsev:2011}.
%remain unavailable for many cases in test and debug. 
The above approaches do not consider the concurrent nature of communication traces of SoC designs, and they rely on temporal dependencies discovered from traces to identify models. However, temporal dependencies are often not the same as the true dependencies that our work aims to find.  


% \marginpar{Till here}
